Large Language Models: New Opportunities for Access to Science

The adaptation of Large Language Models like ChatGPT for information retrieval from scientific data, software and publications is offering new opportunities to simplify access to and understanding of science for persons from all levels of expertise. They can become tools to both enhance the usability of the open science environment we are building as well as help to provide systematic insight to a long-built corpus of scientific publications. The uptake of Retrieval Augmented Generation-enhanced chat applications in the construction of the open science environment of the KM3NeT neutrino detectors serves as a focus point to explore and exemplify prospects for the wider application of Large Language Models for our science.

==> Makefile <==
# Example makefile to help you compile your ADASS proceedings
# but you really should read the ManuscriptInstructions.pdf or
# at least the README file.
# Authors should not need to modify the Makefile, please use the makedefs file, included here
#
# Version 7-oct-2023   Peter Teuben & Tyler Linder/Bob Seaman
#
# See also:   https://www.adass2022.ca/.... / ADASS2022.tar    @todo    for 2023
#
# P = paper_id    your proceedings paper ID code (the one with the XNN syntax, e.g., O12)
# V = version     your version # (1,2,..) since you can only upload unique files
# A = 1stauthor   your last name, e.g. Teuben
# E = email       your contact email for submission issues
# FIGS = *eps     your EPS figures

                    # put your paper_id here (with dash, not dot), e.g. P10-2
                    # or find your template on http://www.astro.umd.edu/~teuben/adass/papers/
P = $(shell ./detect_tex.py | grep -v '^%' | sed 's/.tex//g')
                    # keep incrementing this after each upload of your $(P)
V = 1
                    # First author (for Papercheck.py)
A = Teuben
                    # contact person email
E = teuben@gmail.com
		    # your EPS figures (can be blank, and must be base-named with $(P)_*.eps
FIGS = $(shell ls *.eps)

# override P,V,A,E,FIGS with a "makedefs" file, this is where authors should edit, not this Makefile!!!
-include makedefs

# Which command do you use to view the PDF? This is just for convenience.  (mac uses "open", linux "xdg-open")
# PDFOPEN = xdg-open
PDFOPEN = open

#  variables for proceeding editors (don't modify, for export, not for authors)
YEAR   = 2023
ATDIR  = ADASS$(YEAR)_author_template
FILES  = AdassChecks.py AdassConfig.py AdassIndex.py ADASS_template.tex ADASS_template.pdf \
	 Aindex.py FixUnprintable.py \
	 copyrightform.pdf example.bib example.eps \
	 Index.py manual2010.pdf ManuscriptInstructions.pdf PaperCheck.py \
	 README subjectKeywords.txt TexScanner.py \
	 ascl.py asclKeywords.txt detect_tex.py \
	 adass$(YEAR).bib Makefile makedefs \
	 $(FILESASP)

#  @todo new PID_URL ?
#  probably don't change these either (or notify the editors you have a special paper case)
PID_URL   = "https://www.canfar.net/storage/vault/list/adass2022/upload/$(P)"
TAR_FILE  = $(P).tar.gz
ZIP_FILE  = $(P).zip
POS_FILE  = $(P).pdf
FILESPDF  = $(P).pdf copyrightForm_$(P)_$(A).pdf
FILESTEX  = $(P).tex $(P).bib $(FIGS) makedefs
FILESASP  = asp2014.bst asp2014.sty
FILES4AR  = $(FILESTEX) $(FILESPDF)

# ensure current directory is in the PATH
export PATH := .:$(PATH)

help:
	@echo AUTHOR targets:
	@echo ---------------
	@echo all:   pdf check tar
	@echo pdf:
	@echo check:
	@echo clean:
	@echo overleaf:
	@echo tar:
	@echo zip:
	@echo 
	@echo EDITOR targets:
	@echo ---------------
	@echo fix:
	@echo inc:
	@echo spell:
	@echo aindex:
	@echo words:
	@echo asp1:
	@echo index:   needs TERMS=
	@echo ascl:
	@echo ascl1:
	@echo ascl2:   needs CODE=
	@echo pdf2:
	@echo rsync:


all:	pdf check tar


# not for authors, for creator of the ADASS instruction tar/zip file

aADASS_template.pdf:
	$(MAKE) P=ADASS_template

export: ADASS_template.pdf
	rm -rf $(ATDIR)
	mkdir  $(ATDIR)
	cp -a $(FILES) $(ATDIR)
	echo Created on `date` by `whoami`  > $(ATDIR)/VERSION
	-git remote -v                     >> $(ATDIR)/VERSION
	-git branch                        >> $(ATDIR)/VERSION
	-git rev-list --count HEAD         >> $(ATDIR)/VERSION
	rm -f ADASS$(YEAR).tar ADASS$(YEAR).zip
	tar cf ADASS$(YEAR).tar $(ATDIR)
	zip -urq ADASS$(YEAR).zip $(ATDIR)

# copyright is now part of the tar/zip file, checksum (sum) is 13785
copyrightForm_$(P)_$(A).pdf: copyrightform.pdf
	cp copyrightform.pdf copyrightForm_$(P)_$(A).pdf
	@echo Now go edit your copyrightForm_$(P)_$(A).pdf form

# these targets are for most common unix systems, but YMMV. Modify if you need
# let the editors know you have a better way for the next ADASS team
# ASP prefers the latex;latex;dvipdfm route

DVIPDF = dvipdf

pdf:	$(P).pdf
	@echo $(PDFOPEN) $(P).pdf 

$(P).pdf:  $(P).dvi $(FIGS)
	$(DVIPDF) $(P)

$(P).bib:                                  # bootstrap if you don't have one
	touch $(P).bib

$(P).dvi:  $(P).tex $(P).bib
	latex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	latex $(P)
	latex $(P)

# an alternative method (ASP does not recommend it)
pdflatex:
	pdflatex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	pdflatex $(P)
	pdflatex $(P)

clean:
	rm -f $(P).dvi $(P).bbl $(P).blg $(P).pdf $(P).aux $(P).log $(P).out $(P).toc $(P)_inc.tex

check:
	PaperCheck.py $(P) $(A)

ENCODING =
fix:
	FixUnprintable.py  $(P).tex $(ENCODING)

inc:
	tex2inc.py $(P).tex > $(P)_inc.tex
	@tail -1 $(P)_inc.tex
	@cat $(P).toc

spell:
	aspell --mode=tex --lang=en check $(P).tex
	@echo Share your ~/.aspell.en.pws  ~/.aspell.en.prepl

aspell:
	(cd ../..; $(MAKE) aspell)

dvi:
	latex $(P)

aindex:
	Aindex.py $(P)

DETEX = detex
words:
	$(DETEX) $(P).tex | grep -o -E '\w+' | tr '[A-Z]' '[a-z]' | sort | uniq -c | sort -n

#  could add a checksum on personal copyrightform - if it's 13785,it's bad.
tar:    $(FILES4AR) _checksum
	tar zcf $(TAR_FILE) $(FILES4AR)
	@echo "Login and upload $(TAR_FILE) at $(PID_URL)"

zip:    $(FILES4AR) _checksum
	rm -f $(ZIP_FILE)
	zip $(ZIP_FILE) $(FILES4AR)
	@echo "Login and upload $(ZIP_FILE) at $(PID_URL)"

poster: $(POS_FILE)
	@echo "Login and upload $(POS_FILE) at $(PID_URL)"

overleaf:    $(FILESTEX)
	rm -f $(ZIP_FILE)
	zip $(ZIP_FILE) $(FILESTEX) $(FILESASP)
	@echo You can now upload $(ZIP_FILE) as a new project into overleaf
	@echo After import, git clone this here, and move all the git tree files here.
	@echo "The git clone command is under overleaf's Menu"


_checksum: copyrightForm_$(P)_$(A).pdf
	@echo Checksum test
	@sum copyrightForm_$(P)_$(A).pdf

# for editors
asp1:
	(cd ../..; $(MAKE) asp1 PID=$(P); grep box asp1.log)
	@echo $(PDFOPEN) ../../authors/$(P).pdf

TERMS = foobar
index:
	@echo Using TERMS=$(TERMS)
	(cd ../Author_Template; Index.py $(TERMS))

ssindex:
	@echo Generating ssindex list
	(cd ../Author_Template; ssindex-org.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

ssindex2:
	@echo Generating scored ssindex list 
	(cd ../Author_Template; ssindex-scored.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

index2:
	(cd ../adass_subject_recommender ; detex ../$(P)/$(P).tex |  PYTHONPATH=`pwd` bin/find_subjects.py -m 10 -j)

ascl:
	(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)
# 	(cd ../Author_Template; ascl-new.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

ascl1:
	(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex | grep ooindex | sort | uniq -c)
	-detex $(P).tex > $(P).txt
	-(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).txt | grep ooindex | sort | uniq -c)
	-grep ooindex $(P).tex

CODE = foobar
.PHONY: ascl2
ascl2:
	$(PDFOPEN) https://ascl.net/$(CODE)

pdf2:   pdf asp1
	$(PDFOPEN) $(P).pdf
	$(PDFOPEN) ../../authors/$(P).pdf

rsync: $(P).bib
	rsync -av $(P)_inc.tex $(P).bib $(FIGS) ../../authors
	rm -f ../../authors/$(P)_inc.{bbl,blg}


